MoveTouch: Robotic Motion Capturing System with Wearable Tactile Display to Achieve Safe HRI

The collaborative robot market is flourishing as there is a trend towards simplification, modularity, and increased flexibility on the production line. But when humans and robots are collaborating in a shared environment, the safety of humans should be a priority. We introduce a novel wearable robotic system to enhance safety during Human-Robot Interaction (HRI). The proposed wearable robot is designed to hold a fiducial marker and maintain its visibility to a motion capture system, which, in turn, localizes the user's hand with good accuracy and low latency and provides vibrotactile feedback to the user's wrist. The vibrotactile feedback guides the user's hand movement during collaborative tasks in order to increase safety and enhance collaboration efficiency. A user study was conducted to assess the recognition and discriminability of ten designed vibration patterns applied to the upper (dorsal) and the down (volar) parts of the user's wrist. The results show that the pattern recognition rate on the volar side was higher, with an average of 75.64% among all users. Four patterns with a high recognition rate were chosen to be incorporated into our system. A second experiment was carried out to evaluate users' response to the chosen patterns in real-world collaborative tasks. Results show that all participants responded to the patterns correctly, and the average response time for the patterns was between 0.24 and 2.41 seconds.

==> confusion_down_all_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\centering{
\caption{Confusion matrix for actual and perceived patterns on the volar (down) part of the wrist}
\label{confusion_down_all}
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.95} % Default value: 1
\begin{tabular}{|cc|cccccccccc|}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{10}{c|}{\cellcolor[HTML]{FFFFFF}\textit{Answers   (Predicted Class)}} \\ \hhline{~~----------} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\%}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1H} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}1L} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2H} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}2L} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}3H} &
  \multicolumn{1}{c|}{3L} &
  \multicolumn{1}{c|}{4H} &
  \multicolumn{1}{c|}{4L} &
  \multicolumn{1}{c|}{5H} &
  \multicolumn{1}{c|}{5L} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \cellcolor[HTML]{FFFFFF}1H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5774AA}\color[HTML]{F9FAFB}0.80} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E8ECF4}0.11} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6FA}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \cellcolor[HTML]{FFFFFF}1L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FC}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{345898}\color[HTML]{F9FAFB}0.96} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \cellcolor[HTML]{FFFFFF}2H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{6E87B6}\color[HTML]{F9FAFB}0.69} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E1E6F0}0.15} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6FA}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FC}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FCFCFE}0.02 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \cellcolor[HTML]{FFFFFF}2L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{305496}\color[HTML]{F9FAFB}0.98} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  \cellcolor[HTML]{FFFFFF}3H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{AFBDD7}0.38} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6FA}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{A7B7D3}0.42} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F3F8}0.07} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6FA}0.05} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------} 
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  3L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FC}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6FA}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5371A8}\color[HTML]{F9FAFB}0.82} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{ECF0F6}0.09} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  4H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F3F8}0.07} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E5E9F2}0.13} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{7991BB}\color[HTML]{F9FAFB}0.64} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F3F8}0.07} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F3F8}0.07} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  4L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F3F8}0.07} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E5E9F2}0.13} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5B77AC}\color[HTML]{F9FAFB}0.78} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \cellcolor[HTML]{FFFFFF}0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}} &
  5H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E8ECF4}0.11} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5371A8}\color[HTML]{F9FAFB}0.82} &
  \cellcolor[HTML]{F4F6FA}0.05 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{\multirow{-10}{*}{\cellcolor[HTML]{FFFFFF}\textit{\rotatebox{90}{Patterns}}}} &
  5L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FC}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FC}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FCFCFE}0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D9E0EC}0.18} &
  \cellcolor[HTML]{6E87B6}\color[HTML]{F9FAFB}0.69 \\ \hline

\end{tabular}}
\end{table}

==> confusion_up_all_2.tex <==
%Please add the following required packages to your document preamble:
%\usepackage{multirow}
%\usepackage[table,xcdraw]{xcolor}
%Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

\begin{table}[]
\centering{
\caption{Confusion matrix for actual and perceived patterns on the dorsal (up) part of the wrist}
\label{confusion_up_all}
\setlength{\tabcolsep}{6pt} % Default value: 6pt
\renewcommand{\arraystretch}{0.95} % Default value: 1
\begin{tabular}{|cc|cccccccccc|}
\hline
 
\multicolumn{2}{|c|}{} &
  \multicolumn{10}{c|}{\textit{Answers   (Predicted Class)}} \\ \cline{3-12} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\%}} &
  \multicolumn{1}{c|}{1H} &
  \multicolumn{1}{c|}{1L} &
  \multicolumn{1}{c|}{2H} &
  \multicolumn{1}{c|}{2L} &
  \multicolumn{1}{c|}{3H} &
  \multicolumn{1}{c|}{3L} &
  \multicolumn{1}{c|}{4H} &
  \multicolumn{1}{c|}{4L} &
  \multicolumn{1}{c|}{5H} &
  \multicolumn{1}{c|}{5L} \\ \hline
 
\multicolumn{1}{|c|}{} &
  1H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{40629F}\color[HTML]{F9FAFB}0.87} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F2F7}0.07} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.00} &
  0.00 \\ \hhline{~-----------} 
 
\multicolumn{1}{|c|}{} &
  1L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{305496}\color[HTML]{F9FAFB}0.95} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  0.00 \\ \hhline{~-----------} 
\multicolumn{1}{|c|}{} &
  2H &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5875AB}\color[HTML]{F9FAFB}0.76} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F0F2F7}0.07} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{ECEFF5}0.09} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.00} &
  0.00 \\  \hhline{~-----------}

\multicolumn{1}{|c|}{} &
  2L &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{305496}\color[HTML]{F9FAFB}0.95} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  0.00 \\ \hhline{~-----------}

\multicolumn{1}{|c|}{} &
  3H &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{9CADCD}0.45} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{ACBAD5}0.38} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \cellcolor[HTML]{F8F9FB}0.04 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{} &
  3L &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{647FB1}\color[HTML]{F9FAFB}0.71} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D8DFEB}0.18} &
  \multicolumn{1}{l|}{0.00} &
  0.00 \\ \hhline{~-----------}
\multicolumn{1}{|c|}{} &
  4H &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{B4C1D9}0.35} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{A4B4D1}0.42} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E4E8F1}0.13} &
  0.00 \\ \hhline{~-----------} 
\multicolumn{1}{|c|}{} &
  4L &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D8DFEB}0.18} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{E4E8F1}0.13} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{94A7C9}0.49} &
  \multicolumn{1}{l|}{0.00} &
  \cellcolor[HTML]{F4F6F9}0.05 \\ \hhline{~-----------} 
\multicolumn{1}{|c|}{} &
  5H &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F4F6F9}0.05} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{5472A9}\color[HTML]{F9FAFB}0.78} &
  \cellcolor[HTML]{E4E8F1}0.13 \\ \hhline{~-----------} 
\multicolumn{1}{|c|}{\multirow{-10}{*}{\textit{\rotatebox{90}{Patterns}}}} &
  5L &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{0.00} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{F8F9FB}0.04} &
  \multicolumn{1}{l|}{0.02} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{D4DBE9}0.20} &
  \cellcolor[HTML]{647FB1}\color[HTML]{F9FAFB}0.71 \\ \hline
\end{tabular}}
\end{table}
